The non-overlapping statistical approximation to overlapping group lasso

Group lasso is a commonly used regularization method in statistical learning in which parameters are eliminated from the model according to predefined groups. However, when the groups overlap, optimizing the group lasso penalized objective can be time-consuming on large-scale problems because of the non-separability induced by the overlapping groups. This bottleneck has seriously limited the application of overlapping group lasso regularization in many modern problems, such as gene pathway selection and graphical model estimation. In this paper, we propose a separable penalty as an approximation of the overlapping group lasso penalty. Thanks to the separability, the computation of regularization based on our penalty is substantially faster than that of the overlapping group lasso, especially for large-scale and high-dimensional problems. We show that the penalty is the tightest separable relaxation of the overlapping group lasso norm within the family of $\ell_{q_1}/\ell_{q_2}$ norms. Moreover, we show that the estimator based on the proposed separable penalty is statistically equivalent to the one based on the overlapping group lasso penalty with respect to their error bounds and the rate-optimal performance under the squared loss. We demonstrate the faster computational time and statistical equivalence of our method compared with the overlapping group lasso in simulation examples and a classification problem of cancer tumors based on gene expression and multiple gene pathways.

==> Generlizaiton.tex <==
\section{More theoretical results}
To extend our result for user-defined group weights, we provide the generalized version of our results in this section. We add $\ast$ to the result to indicate that this is the generalized version. For example, theorem $1^{\ast}$ is the generalized version of   theorem $1$ 




\ref{pro1}
$\phi^{\ast}$, the dual norm of overlapping penalty in equation (\ref{a}), is defined as:
 \begin{equation}
     \phi^{\ast}(\beta)=\max\limits_{g\in\{1,\cdots,m\}}\frac{1}{w_g}\left\|(H\beta)_{G_g}\right\|_2,
 \end{equation}
 where $H = diag(\frac{1}{h_1},\cdots,\frac{1}{h_p})$ is a diagonal matrix.


==> Group_Lasso.tex <==
\section{Methodology}
\label{sec:methods}
\paragraph{Notation and Preliminaries.} Throughout this paper,  for any integer $z$, we use $[z]$ to denote the index set $\{1,\cdots,z\}$. For two sequences $\{a_n\}$ and $\{b_n\}$, we write  $a_n \ll b_n$ if $a_n = o(b_n)$, write $a_n \lesssim b_n$ if $a_n \leqslant Cb_n$ for a sufficiently large $n$ and a universal constant $C > 0$, and write $a_n \asymp b_n$ if $a_n \lesssim b_n$ and $a_n \gtrsim b_n$ both hold. For a set $T$, we use $|T|$ to denote the cardinal number of $T$. For a matrix $A$, we use $A_{T}$ to denote the sub-matrix of $A$  consisting of the columns indexed by the set $T$, and  use $A_{T,T}$  to denote the sub-matrix of $A$ consisting of both rows and columns indexed by the set $T$.  When $A$ is a symmetric matrix, we use $\gamma_{\min}(A)$ and $\gamma_{\max}(A)$ to denote the smallest and the largest eigen-values of $A$. We introduce other notations in context, and summarize all notations used in Table~\ref{tab:notations} of Appendix~\ref{sec:notations}.


\subsection{Group Lasso}
Suppose that the parameters in our model are represented by a vector $\beta \in \mathbb{R}^p$ for which $\beta_j$ denotes the $j$-th element of $\beta$. Let $G = \{G_1,\cdots,G_m\}$ be the $m$ predefined groups for the $p$ parameters, that is, each group $G_g$ is a subset of $[p]$, and $\cup_{k\in [p]}G_k = [p]$. For each group $G_g$, we use $d(G)_g = |G_g|$ to denote the group size, and abbreviate it by $d_g$ when the group structure is clear in context. Given $G_g$, we let $\beta_{G_g}$ denote the a subvector of  $\beta$ indexed by $G_g$. Additionally, we could have user-defined positive weights $w = \{w_1,\cdots,w_m\}$ associated with each group. The group lasso norm \citep{yuan2006model} is defined as

\begin{equation}
\label{eq:glnorm}
    \phi_G(\beta)  = \sum\limits_{g \in [m]}{w_g \left\|\beta_{G_g}\right\|_2,}
\end{equation}
where the weights are usually set to be $1$ or $\sqrt{d_g}$ in applications. When the group $G$ is clear, we may suppress $G$ and write $\phi_G(\beta)$ as $\phi(\beta)$

In statistical estimation problems involving group selection, the group lasso norm is combined with an empirical loss function $L_n$, and the estimator $\beta^\ast$ is solved by the following M-estimation problem.

\begin{equation}
\label{glreg}
    \hat{\beta}^{G} =\arg\min\limits_{\beta\in  \mathbb{R}^p}\left\{ L_n(\beta) +\lambda_n\phi(\beta)\right\},
\end{equation} 
When groups overlap, the group lasso leads to solutions whose nonzero support is contained in the complement to a union of groups \citep{ogl,wainwright2019high}, with a possibility that some groups may have partial zeros. Such a pattern is desired in many problems such as graph structure recovery and structure learning \citep{tcap,ogl, hmgm,mohan2014node,tarzanagh2018estimation}. Yet another generalization of the group lasso aims to partially eliminate parts of some groups while maintaining full nonzero in other groups; this is called the latent overlapping group lasso \citep{ogl}. This method is suitable in a set of different applications \citep{hvs,bien2018graph} and is not our focus in this paper.
%%%%%%%%%%%%%%%%%%%%%
% P1: Introduce dual method
%%%%%%%%%%%%%%%%%%%%%

Problem~\eqref{glreg} is a non-smooth convex optimization problem, and the proximal gradient method \citep{nesterov2013gradient,beck2009fast} is one of the most general yet efficient strategies to solve it. Intuitively, proximal gradient descent minimizes the objective iteratively by applying the proximal operator of $\lambda_n\phi(\beta)$ at each step.  The proximal operator associated with group lasso penalty in \eqref{eq:glnorm} is defined as
\begin{equation}
\label{op}
    \mathop\mathrm{argmin}_{\beta\in \mathbb{R}^p}\frac{1}{2}|| \mu - \beta ||^2 + \lambda_n \phi_G(\beta).
\end{equation}
As studied in \citet{svsw}, the dual of the proximal operator \eqref{op} is%(\ref{op}) \TL{Look at my LaTex source to see how to correctly make reference. You use eqref rather than eq for formula} with strong dual is given by 
 \begin{equation}
 \label{opp}
    \mathop\mathrm{minimize}_{\{\xi^g\in \mathbb{R}^p\}_{g \in [m]}}\left(\frac{1}{2}|| \mu - \sum_{g=1}^m \xi^g||^2_2 \right), \hspace{0.5cm} s.t \hspace{0.2cm}||\xi^g||_2 \leq \lambda_n w_g \hspace{0.2cm} \textit{and} \hspace{0.2cm} \xi^g_j \neq 0 \hspace{0.2cm}\textit{if} \hspace{0.2cm} j \notin G_g.
\end{equation}
\citet{svsw} proposed to solve the proximal operator of the group lasso penalty by a block coordinate descent (BCD) algorithm (see Algorithm~\ref{alg1}).  \citet{ES} and \citet{chen2012smoothing} further smoothed %\eqref{opp}
proximal gradient procedure to improve its efficiency. For completeness, Proposition~\ref{pro2} guarantees the convergence property of
%algorithm
 Algorithm~\ref{alg1}.%(\ref{opp}). 
 
 {\tiny
   \begin{algorithm}[hbt]
    \caption{BCD algorithm for the proximal
operator of group lasso penalty}
    \label{alg1}
    \hspace*{\algorithmicindent} \textbf{Input: $\mathbf{G},$ $\left\{w_g\right\}_{g=1}^m$,  $u$, $\lambda_n$, } \\
    \hspace*{\algorithmicindent} \textbf{Requirement:}  $\mathbf{G}$, $\left\{w_g\right\}_{g=1}^m > 0$,  $\lambda_n > 0$.\\
    \hspace*{\algorithmicindent} \textbf{Initialization: Set $\left\{\xi^{g}\right\}_{g=1}^m = 0 \in \mathbb{R}^p.$ } \\
    \hspace*{\algorithmicindent} \textbf{Output: $\beta^\ast$ } 
     \begin{algorithmic}[1]
     \While {stopping criterion not reached} 
         \ForAll{$g\in \{1, \cdots,m \}$}
         \State Calculate $r^g = \mu - \sum_{h \neq g} \xi^h$.
      \If{$||r^g||_2 \leqslant \lambda_n  w_g$}~~
     $ \xi_j^g  = \begin{cases*}
                    0 & if  $j \notin G_g$  \\
                   r_j^g & if  $j \in G_g$ 
                 \end{cases*} $
    \Else~~
     $\xi_j^g  = \begin{cases*}
                    0 & if  $j \notin g$  \\
                   \frac{\lambda  w_gr_j^{g}}{||r^{g}||_2} & if  $j \in G_g$ 
                 \end{cases*} $
    \EndIf
  \EndFor
	     	\EndWhile
    \State $\beta^\ast = u - \sum\limits_{g = 1}^{m}\xi^{g}.$
    \end{algorithmic}
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%%%
% P2: Convergence of dual method
%%%%%%%%%%%%%%%%%%%%%
\begin{pro}
\label{pro2}
The cluster point generated iterations in Algorithm~\ref{alg1} achives the global minimum of the problem \eqref{opp}.
\end{pro}


%%%%%%%%%%%%%%%%%%%%%
% P3: Computational time of dual method vs. group lasso
%%%%%%%%%%%%%%%%%%%%%


Even if algorithms other than proximal+BCD are used to solve \eqref{glreg}, the formulation of \eqref{op} and \eqref{opp} still delivers insights about the bottleneck caused by the overlapping groups. The overlapping groups make the penalty non-separable between variables, compared to its non-overlapping counterpart. The duality between \eqref{op} and \eqref{opp} shows that the overlapping group lasso problem has an intrinsic dimension equal to a $\sum_{g \in [m]} d_g$-dimensional separable problem. When the groups have a nontrivial proportion of overlapping variables, the computation of the overlapping group lasso becomes substantially more diﬃcult, eventually prohibitive on large-scale problems.
This issue significantly limits the applicability of the group lasso penalty in overlapping problems. Next, we introduce our non-overlapping approximation as a solution to this rectify this challenge.



\subsection{Non-overlapping Approximation of the Overlapping Group Lasso}

Given that the crux lies in the non-separability of parameters, the key to improving the computation is to introduce separable operators. We first use a special interlocking group structure to illustrate our idea. In an interlocking group structure, groups are ordered and each group overlaps with its neighbors (see Figure~\ref{fig_OG}). We assume $w_g \equiv 1$  in this example for simplicity.
\begin{figure}[H]
\centering
     \begin{subfigure}[t]{0.75\textwidth}
         \centering
         \includegraphics[width=\textwidth]{int1.png}
         \caption{Illustration of interlocking  group structure.}
         \label{fig_OG}
     \end{subfigure}
     
     \vspace*{1cm}
     \begin{subfigure}[t]{0.75\textwidth}
         \centering
         \includegraphics[width=\textwidth]{int2.png}
         \caption{Illustration of partitioned group structure.}
         \label{fig_nonOG}
     \end{subfigure}
\caption{Illustration of proposed group partition in an interlocking group structure. Red regions are the overlapping variables in the original group structure. }
\label{figillu}
\end{figure}



We introduce a new group partition of the variables, as in Figure~\ref{fig_nonOG}, which precisely separates the intersections as separable groups. We denote the new groups as $\Gcal = \{\Gcal_1, \cdots, \Gcal_\mcal\}$, and in this particular case, $\mcal = 2m-1$. By triangular inequality we have
$$\norm{\beta_{G_1}}_2 \le \norm{\beta_{\Gcal_1}}_2 + \norm{\beta_{\Gcal_2}}_2.$$
With similar inequalities applied to each item, the overlapping group lasso norm based on $G$ can be controlled by a reweighted non-overlapping group norm based on $\Gcal$ as
\begin{equation}\label{eq:demo-ineq}
\sum\limits_{g \in [m]}{\norm{\beta_{G_g}}_2} \le \sum_{\gcal \in [\mcal]}\hcal_\gcal\norm{\beta_{\Gcal_{\gcal}}}_2%\left\|\beta_{\Gcal_1}\right\|_2 + \sum\limits_{2 \le \gcal \le 2m-2}{2\left\|\beta_{\Gcal_g}\right\|_2} +  \norm{\beta_{\Gcal_{2m-1}}}_2
\end{equation}
where $\hcal_{\gcal} = 1$ for odd numbers $\gcal$ and $2$ for even numbers $\gcal$. That is, controlling the right side of \eqref{eq:demo-ineq} is suﬃcient to control the overlapping group norm on the left side. The advantage, however, is that the right-side norm is separable and allows for eﬃcient optimization.



%\TL{I wrote the macro $\backslash$norm\{\} for you. You can use it anywhere you need the norm notation in the future. Can't imagine how much time you have wasted in writing using the previous one...}


This idea is indeed applicable for general overlapping group structure $G$. The pre-defined group $G$ can be represented by a $m\times p$ binary matrix $\mathbf{G}$, where $\mathbf{G}_{gj}=1$ if and only if  the $j$-th variable belongs to the $g$-th group. 

Our approximation starts from finding a partition of the $p$ variables by grouping identical columns in  $\Gbf$, and we denote this new partition as $\Gcal$. To be more specific, if  $\mathbf{G}_{,j_1} = \mathbf{G}_{,j_2}$, then the $j_1\text{th}$ variable and the $j_2\text{th}$ variable are partitioned into the same group in $\Gcal$. Note that the groups $\Gcal$ are disjoint by this definition. All quantities such as number of groups and group sizes can be similarly defined for $\Gcal$. To distinguish $G$ and $\Gcal$ while maintaining the connection between the quantities, we use normal letters, such as $\{g,d,m,w,G\}$, to denote quantities about  the original group structure, and use calligraphic letters, such as $\{\mathcal{g,d,m,w,G}\}$, as notations about the group structure in the induced non-overlapping groups. For example, $\mcal$ is the number of groups in $\Gcal$ and $\gcal \in [\mcal]$ is used as the index of groups in $\Gcal$.

Each group $\mathcal{G}_\mathcal{g} \in \Gcal$ is a subset for some groups in $G$. Define
$$F(\mathcal{g}) = \{g: g\in [m], \Gcal_{\gcal} \subset G_g \} ~~~~\text{and}~~~~F^{-1}(g) = \{\gcal: \gcal\in [\mcal], \Gcal_{\gcal} \subset G_g\}.
$$
%Similarly, for  $G_g \in G$, we use $F^{-1}(g) \subseteq [\mathcal{m}]$ to denote the non-overlapping groups in $\Gcal$ that partition from $G_g$. 
In addition, we define the overlapping degree of each variable $j$ as $h_j(\mathbf{G}) = \sum_{g \in [m]}\mathbf{G}_{gj}$, and define $h_{\max}(\mathbf{G}) = \max_{j \in [p]}h_j(\mathbf{G})$. Notice that all variables in the same $\mathcal{G}_\mathcal{g}$ have the same overlapping degree by definition, denoted as $\mathcal{h}_{\mathcal{g}} = h_{\text{\{}j|j \in \mathcal{G}_{\mathcal{g}}\text{\}}}$. In the previous example of the interlocking groups, we have $h_g$ is either 1 or 2 and $h_{\max} = 2$ in $G$.

Given positive weights $w$ of $G$, we proposed to set the weight $\mathcal{w}$ of $\mathcal{G}$ by 
$$\mathcal{w}_\mathcal{g} =  \sum_{g\in F(\mathcal{g}) }w_g, \gcal \in [\mcal].$$ 

With the new partition $\Gcal$ and the new weights $\wcal$, we fine the following norm as the separable alternative of  overlapping group lasso norm. 
\begin{equation}\label{eq:our-norm}
\psi_{\Gcal}(\beta) = \sum\limits_{\mathcal{g}=1}^{\mathcal{m}}{\mathcal{w}_{\mathcal{g}}\left\|\beta_{\mathcal{G}_g}\right\|_2}. 
 \end{equation}

In general, by triangular inequality, the proposed norm is always an upper bound of the original group lasso norm:
\begin{equation}\label{eq:general-ineq}
\phi_G(\beta) = \sum\limits_{g=1}^{m}{w_g\left\|\beta_{G_g}\right\|_2} \leqslant \sum\limits_{\mathcal{g}=1}^{\mathcal{m}}{\mathcal{w}_{\mathcal{g}}\left\|\beta_{\mathcal{G}_g}\right\|_2} = \psi_{\Gcal}(\beta).
\end{equation}
Our proposed penalty is essentially a weighted non-overlapping group lasso on $\Gcal$. For illustration, Figure \ref{cof} shows the unit ball of these two norms based on $G_1 = \{\beta_1, \beta_2 \}$ and $G_2 = \{\beta_1 ,\beta_2, \beta_3 \}$. All singular points of the $\phi_G$-ball (where exactly zero happens in optimization) are also singular points of the $\psi_{\Gcal}$-ball. 


\begin{figure}[H]
     \centering    
          \vspace{-3cm}
        \includegraphics[width=0.6\textwidth]{Fig1.pdf}
         \vspace{-3cm}
 \caption {Outside: unit ball of the overlapping group lasso norm $\{ \beta: \sqrt{ \beta_1^2 + \beta_2^2 } +  \sqrt{ \beta_1^2 + \beta_2^2 + \beta_3^2 }  \leqslant 1 \}$; Inside: unit ball of our proposed separable norm $\{ \beta: 2\sqrt{ \beta_1^2 + \beta_2^2 } +  \sqrt{ \beta_3^2 }  \leqslant 1 \}$.}
        \label{cof}
\end{figure}

Readers might notice that \eqref{eq:general-ineq} can hold for other separable norms as well. For example, we can split all $p$ variables into separate groups and use a weighted lasso norm 
 \begin{equation}\label{eq:weighted-lasso}
 \sum\limits_{j=1}^{p}{\left(\sum_{\{g|\beta_j \in G_g\} }w_g\right)\left|\beta_j\right|} 
 \end{equation}
% 
 as another upper bound of $\phi_G$, which is the strategy of  \cite{hmgm}. 
 So what is special about the proposed norm in \eqref{eq:our-norm}? 
 
 Intuitively, as can be seen from our construction procedure for $\Gcal$, or Figure~\ref{cof}, our construction only introduces additional singular points for the norm when it is necessary to achieve separability. Compared with using a lasso upper bound, our procedure does not introduce redundancy in addition to the separability. Therefore, our approximation should achieve certain tightness. 
 %For example, note that we have
 %$$\phi_G(\beta) \le \psi_{\Gcal}(\beta) \le \sum\limits_{j=1}^{p}{\left(\sum_{\{g|\beta_j \in G_g\} }w_g\right)\left|\beta_j\right|}.$$
 %So our $\psi_{\Gcal}$ is always a tighter approximation than the weight lasso. \
 Next, we rigorously verify the above intuition in a formal way. Specifically, given any group structure $G$ and weights $w$, we define the $\ell_{q_1}/\ell_{q_2} $ norm of $\beta$ for any $0 \leqslant q_1,q_2 \leqslant \infty$ as
\begin{equation}
\label{gnorm}
||\beta_{\{G,w\}}||_{q_1,q_2} = \left(\sum\limits_{g \in [m]}w_g||\beta_{G_g}||_{q_2}^{q_1}\right)^\frac{1}{q_1}
    = \left\{ \sum\limits_{g \in [m]} w_g\left( \sum\limits_{j \in G_g}|\beta_j|^{q_2}\right)^{\frac{q_1}{q_2}}\right\}^{\frac{1}{q_1}}.
\end{equation}
This is a general class of norms that potentially includes most of the penalties that are reasonable use in the current context.  In particular, it includes the weighted lasso penalty.  The following theorem shows that the proposed norm is the \emph{tightest separable relaxation} of the original overlapping group lasso norm among all separable $\ell_{q_1}/\ell_{q_2}$ norms.

\begin{theorem}
\label{addtheo}
Given the original weight $w$, let $\mathbb{G}$ be the space of all possible partitions of $[p]$, then there does not exist  $0 \leqslant q_1,q_2 \leqslant \infty, \tilde{G} \in \mathbb{G}, \tilde{w} \in [0, \infty)^p,$ such that 
\begin{equation}
    \label{twocondi}
    \begin{cases}
 \sum\limits_{g\in [m]}w_g||\beta_{G_g}||_2 \leqslant ||\beta_{\{\tilde{G},\tilde{w}\}}||_{q_1,q_2} \leqslant \sum\limits_{\mathcal{g} \in [\mathcal{m}]}\mathcal{w}_\mathcal{g}||\beta_{\mathcal{G}_\mathcal{g}}||_2  &  \text{ for all $\beta \in \mathbb{R}^p$} \\
  ||\beta_{\{\tilde{G},\tilde{w}\}}||_{q_1,q_2} < \sum\limits_{\mathcal{g} \in [\mathcal{m}]}\mathcal{w}_\mathcal{g}||\beta_{\mathcal{G}_\mathcal{g}}||_2  &  \text{ for some $\beta \in \mathbb{R}^p$}
\end{cases}.
\end{equation}
\end{theorem}





%In terms of the common setting where  $w_g \asymp \sqrt{d_g},$  we propose to modify the group weights for the partition groups by setting $\mathcal{w}_\mathcal{g} \asymp \sum\limits_{g\in F(\mathcal{g}) } \sqrt{d_g}.$ In terms of the setting where  $w_g \asymp 1,$ we propose to set the partitioned group weights as  $\mathcal{w}_\mathcal{g} \asymp  \mathcal{h}_\mathcal{g}.$ For user-defined weight settings, we provide a general rule in the following section.
%\TL{I don't understand this paragraph. In the discussions below and my understanding of your current writing, you only talk about unweighted cases the property until Theorem 1, correct? Then why should you talk about $w_g$ at this part? Perhaps it is easier to move it to the end of the section when you finally define the version for general weights? Also, this part is supposed to give definition or practical guidance. So we cannot say something like $w_g\asymp \sqrt{d}$. We have to define them exactly, so people can follow your definition to specify thing in their programs. }

